Interpersonal Trust Among Students in Virtual Learning Environments: A Comprehensive Review

Interpersonal trust is recognized as one of the pillars of collaboration and successful learning among students in virtual learning environments (VLEs). This systematic mapping study investigates attributes, phases, and features that support interpersonal trust among students in VLEs. Analyzing 46 articles, we identified 37 attributes that influence phases of acquiring and losing trust, categorized into four themes: Ability, Integrity, Affinity, and Non-Personal Factors. Attributes such as collaborative and ethical behavior, academic skills, and higher grades are often used to select peers, mainly through recommendation systems and user profiles. To organize our findings, we elaborated two conceptual maps describing the main characteristics of trust definitions and the attributes classification by phases and themes.

==> Highlights.tex <==
\begin{highlights}
\item Trust-based relationships are grounded on student affinity, integrity, and ability
\item Affinity with other students is the main factor considered in a recommendation
\item Recommendation systems are used to identify trustworthy peers
\item Communication and collaboration features are key to building initial trust
\end{highlights}
